Error Decoding of Locally Repairable and Partial MDS Codes

In this work it is shown that locally repairable codes (LRCs) can be list-decoded efficiently beyond the Johnson radius for a large range of parameters by utilizing the local error-correction capabilities. The corresponding decoding radius is derived and the asymptotic behavior is analyzed. A general list-decoding algorithm for LRCs that achieves this radius is proposed along with an explicit realization for LRCs that are subcodes of Reed--Solomon codes (such as, e.g., Tamo--Barg LRCs). Further, a probabilistic algorithm of low complexity for unique decoding of LRCs is given and its success probability is analyzed. The second part of this work considers error decoding of LRCs and partial maximum distance separable (PMDS) codes through interleaved decoding. For a specific class of LRCs the success probability of interleaved decoding is investigated. For PMDS codes, it is shown that there is a wide range of parameters for which interleaved decoding can increase their decoding radius beyond the minimum distance such that the probability of successful decoding approaches $1$ when the code length goes to infinity.

==> points_PMDS.tex <==
\addplot [only marks, mark=diamond*, color=blue] table {
0.030000 0.270000
0.030000 0.310000
0.030000 0.370000
0.030000 0.410000
0.030000 0.430000
0.030000 0.610000
0.030000 0.670000
0.030000 0.750000
0.050000 0.310000
0.050000 0.350000
0.050000 0.370000
0.050000 0.390000
0.050000 0.410000
0.050000 0.430000
0.050000 0.450000
0.050000 0.550000
0.050000 0.570000
0.050000 0.610000
0.050000 0.630000
0.050000 0.670000
0.050000 0.710000
0.050000 0.750000
0.050000 0.810000
0.050000 0.830000
0.070000 0.350000
0.070000 0.370000
0.070000 0.390000
0.070000 0.430000
0.070000 0.450000
0.070000 0.470000
0.070000 0.530000
0.070000 0.550000
0.070000 0.570000
0.070000 0.590000
0.070000 0.610000
0.070000 0.630000
0.070000 0.670000
0.070000 0.710000
0.070000 0.750000
0.070000 0.770000
0.070000 0.810000
0.070000 0.830000
0.070000 0.850000
0.070000 0.870000
0.090000 0.350000
0.090000 0.390000
0.090000 0.450000
0.090000 0.470000
0.090000 0.530000
0.090000 0.550000
0.090000 0.570000
0.090000 0.590000
0.090000 0.610000
0.090000 0.630000
0.090000 0.650000
0.090000 0.690000
0.090000 0.710000
0.090000 0.730000
0.090000 0.750000
0.090000 0.770000
0.090000 0.810000
0.090000 0.830000
0.090000 0.850000
0.090000 0.870000
0.090000 0.890000
0.090000 0.910000
0.110000 0.390000
0.110000 0.450000
0.110000 0.470000
0.110000 0.530000
0.110000 0.550000
0.110000 0.570000
0.110000 0.590000
0.110000 0.610000
0.110000 0.630000
0.110000 0.650000
0.110000 0.690000
0.110000 0.710000
0.110000 0.730000
0.110000 0.750000
0.110000 0.770000
0.110000 0.790000
0.110000 0.810000
0.110000 0.830000
0.110000 0.850000
0.110000 0.870000
0.110000 0.890000
0.110000 0.910000
0.130000 0.450000
0.130000 0.470000
0.130000 0.490000
0.130000 0.530000
0.130000 0.550000
0.130000 0.570000
0.130000 0.590000
0.130000 0.610000
0.130000 0.630000
0.130000 0.650000
0.130000 0.690000
0.130000 0.710000
0.130000 0.730000
0.130000 0.750000
0.130000 0.770000
0.130000 0.790000
0.130000 0.810000
0.130000 0.830000
0.130000 0.850000
0.130000 0.870000
0.130000 0.890000
0.130000 0.910000
0.130000 0.930000
0.150000 0.470000
0.150000 0.530000
0.150000 0.550000
0.150000 0.570000
0.150000 0.590000
0.150000 0.610000
0.150000 0.630000
0.150000 0.650000
0.150000 0.690000
0.150000 0.710000
0.150000 0.730000
0.150000 0.750000
0.150000 0.770000
0.150000 0.790000
0.150000 0.810000
0.150000 0.830000
0.150000 0.850000
0.150000 0.870000
0.150000 0.890000
0.150000 0.910000
0.150000 0.930000
0.170000 0.470000
0.170000 0.490000
0.170000 0.530000
0.170000 0.550000
0.170000 0.570000
0.170000 0.590000
0.170000 0.610000
0.170000 0.630000
0.170000 0.650000
0.170000 0.690000
0.170000 0.710000
0.170000 0.730000
0.170000 0.750000
0.170000 0.770000
0.170000 0.790000
0.170000 0.810000
0.170000 0.830000
0.170000 0.850000
0.170000 0.870000
0.170000 0.890000
0.170000 0.910000
0.170000 0.930000
0.170000 0.950000
0.190000 0.470000
0.190000 0.490000
0.190000 0.530000
0.190000 0.550000
0.190000 0.570000
0.190000 0.590000
0.190000 0.610000
0.190000 0.630000
0.190000 0.650000
0.190000 0.690000
0.190000 0.710000
0.190000 0.730000
0.190000 0.750000
0.190000 0.770000
0.190000 0.790000
0.190000 0.810000
0.190000 0.830000
0.190000 0.850000
0.190000 0.870000
0.190000 0.890000
0.190000 0.910000
0.190000 0.930000
0.190000 0.950000
0.210000 0.490000
0.210000 0.530000
0.210000 0.550000
0.210000 0.590000
0.210000 0.610000
0.210000 0.630000
0.210000 0.650000
0.210000 0.690000
0.210000 0.710000
0.210000 0.730000
0.210000 0.770000
0.210000 0.790000
0.210000 0.810000
0.210000 0.830000
0.210000 0.850000
0.210000 0.870000
0.210000 0.890000
0.210000 0.910000
0.210000 0.930000
0.210000 0.950000
0.230000 0.550000
0.230000 0.590000
0.230000 0.630000
0.230000 0.650000
0.230000 0.690000
0.230000 0.710000
0.230000 0.730000
0.230000 0.770000
0.230000 0.790000
0.230000 0.810000
0.230000 0.830000
0.230000 0.850000
0.230000 0.870000
0.230000 0.890000
0.230000 0.910000
0.230000 0.930000
0.230000 0.950000
0.250000 0.590000
0.250000 0.630000
0.250000 0.650000
0.250000 0.690000
0.250000 0.710000
0.250000 0.730000
0.250000 0.770000
0.250000 0.790000
0.250000 0.810000
0.250000 0.830000
0.250000 0.850000
0.250000 0.870000
0.250000 0.890000
0.250000 0.910000
0.250000 0.930000
0.250000 0.950000
0.250000 0.970000
0.270000 0.590000
0.270000 0.650000
0.270000 0.690000
0.270000 0.710000
0.270000 0.730000
0.270000 0.770000
0.270000 0.790000
0.270000 0.810000
0.270000 0.830000
0.270000 0.850000
0.270000 0.870000
0.270000 0.890000
0.270000 0.910000
0.270000 0.930000
0.270000 0.950000
0.270000 0.970000
0.290000 0.650000
0.290000 0.690000
0.290000 0.710000
0.290000 0.730000
0.290000 0.770000
0.290000 0.790000
0.290000 0.810000
0.290000 0.830000
0.290000 0.850000
0.290000 0.870000
0.290000 0.890000
0.290000 0.910000
0.290000 0.930000
0.290000 0.950000
0.310000 0.690000
0.310000 0.710000
0.310000 0.730000
0.310000 0.770000
0.310000 0.790000
0.310000 0.830000
0.310000 0.850000
0.310000 0.870000
0.310000 0.890000
0.310000 0.910000
0.310000 0.930000
0.310000 0.950000
0.330000 0.650000
0.330000 0.690000
0.330000 0.710000
0.330000 0.730000
0.330000 0.770000
0.330000 0.790000
0.330000 0.830000
0.330000 0.850000
0.330000 0.870000
0.330000 0.890000
0.330000 0.910000
0.330000 0.930000
0.330000 0.970000
0.350000 0.650000
0.350000 0.690000
0.350000 0.710000
0.350000 0.730000
0.350000 0.770000
0.350000 0.790000
0.350000 0.830000
0.350000 0.850000
0.350000 0.870000
0.350000 0.890000
0.350000 0.910000
0.350000 0.930000
0.350000 0.950000
0.370000 0.690000
0.370000 0.730000
0.370000 0.770000
0.370000 0.790000
0.370000 0.830000
0.370000 0.850000
0.370000 0.870000
0.370000 0.890000
0.370000 0.910000
0.370000 0.930000
0.370000 0.950000
0.370000 0.970000
0.390000 0.690000
0.390000 0.730000
0.390000 0.770000
0.390000 0.790000
0.390000 0.850000
0.390000 0.870000
0.390000 0.890000
0.390000 0.910000
0.390000 0.930000
0.390000 0.950000
0.390000 0.970000
0.410000 0.690000
0.410000 0.770000
0.410000 0.850000
0.410000 0.870000
0.410000 0.890000
0.410000 0.910000
0.410000 0.930000
0.410000 0.950000
0.410000 0.970000
0.430000 0.770000
0.430000 0.790000
0.430000 0.850000
0.430000 0.870000
0.430000 0.890000
0.430000 0.910000
0.430000 0.930000
0.430000 0.950000
0.450000 0.770000
0.450000 0.790000
0.450000 0.870000
0.450000 0.890000
0.450000 0.910000
0.470000 0.770000
0.470000 0.790000
0.470000 0.870000
0.470000 0.890000
0.470000 0.910000
0.470000 0.930000
0.470000 0.950000
0.490000 0.790000
0.490000 0.870000
0.490000 0.890000
0.490000 0.910000
0.490000 0.930000
0.490000 0.970000
0.490000 0.990000
0.510000 0.790000
0.510000 0.890000
0.510000 0.910000
0.510000 0.930000
0.510000 0.950000
0.530000 0.890000
0.530000 0.910000
0.530000 0.930000
0.530000 0.950000
0.550000 0.890000
0.550000 0.910000
0.550000 0.930000
0.550000 0.950000
0.550000 0.970000
0.570000 0.890000
0.570000 0.910000
0.570000 0.930000
0.570000 0.950000
0.570000 0.970000
0.590000 0.910000
0.590000 0.930000
0.590000 0.950000
0.590000 0.970000
0.610000 0.930000
0.610000 0.950000
0.610000 0.970000
0.630000 0.930000
0.630000 0.950000
0.650000 0.930000
0.650000 0.950000
0.650000 0.970000
0.650000 0.990000
0.670000 0.930000
0.670000 0.950000
0.690000 0.930000
0.690000 0.950000
0.690000 0.970000
0.710000 0.950000
0.730000 0.950000
0.730000 0.970000
0.730000 0.990000
0.750000 0.950000
0.770000 0.970000
0.790000 0.970000
0.810000 0.970000
0.830000 0.970000
};

==> points_both.tex <==
\addplot [only marks, mark=triangle*, color=mygreen] table {
0.030000 0.090000
0.030000 0.110000
0.030000 0.130000
0.030000 0.150000
0.030000 0.170000
0.030000 0.190000
0.030000 0.210000
0.030000 0.230000
0.030000 0.250000
0.030000 0.290000
0.030000 0.330000
0.030000 0.510000
0.050000 0.110000
0.050000 0.130000
0.050000 0.150000
0.050000 0.170000
0.050000 0.190000
0.050000 0.210000
0.050000 0.230000
0.050000 0.250000
0.050000 0.270000
0.050000 0.290000
0.050000 0.330000
0.050000 0.510000
0.070000 0.130000
0.070000 0.150000
0.070000 0.170000
0.070000 0.190000
0.070000 0.210000
0.070000 0.230000
0.070000 0.250000
0.070000 0.270000
0.070000 0.290000
0.070000 0.310000
0.070000 0.330000
0.070000 0.410000
0.070000 0.510000
0.090000 0.170000
0.090000 0.190000
0.090000 0.210000
0.090000 0.230000
0.090000 0.250000
0.090000 0.270000
0.090000 0.290000
0.090000 0.310000
0.090000 0.330000
0.090000 0.370000
0.090000 0.410000
0.090000 0.430000
0.090000 0.510000
0.090000 0.670000
0.110000 0.210000
0.110000 0.230000
0.110000 0.250000
0.110000 0.270000
0.110000 0.290000
0.110000 0.310000
0.110000 0.330000
0.110000 0.350000
0.110000 0.370000
0.110000 0.410000
0.110000 0.430000
0.110000 0.510000
0.110000 0.670000
0.130000 0.190000
0.130000 0.210000
0.130000 0.250000
0.130000 0.270000
0.130000 0.290000
0.130000 0.310000
0.130000 0.330000
0.130000 0.350000
0.130000 0.370000
0.130000 0.390000
0.130000 0.410000
0.130000 0.430000
0.130000 0.510000
0.130000 0.670000
0.150000 0.210000
0.150000 0.230000
0.150000 0.290000
0.150000 0.310000
0.150000 0.330000
0.150000 0.350000
0.150000 0.370000
0.150000 0.390000
0.150000 0.410000
0.150000 0.430000
0.150000 0.450000
0.150000 0.510000
0.150000 0.670000
0.170000 0.250000
0.170000 0.270000
0.170000 0.290000
0.170000 0.330000
0.170000 0.350000
0.170000 0.370000
0.170000 0.390000
0.170000 0.410000
0.170000 0.430000
0.170000 0.450000
0.170000 0.510000
0.170000 0.670000
0.190000 0.270000
0.190000 0.290000
0.190000 0.310000
0.190000 0.330000
0.190000 0.370000
0.190000 0.390000
0.190000 0.410000
0.190000 0.430000
0.190000 0.450000
0.190000 0.510000
0.190000 0.670000
0.210000 0.310000
0.210000 0.330000
0.210000 0.350000
0.210000 0.370000
0.210000 0.390000
0.210000 0.410000
0.210000 0.430000
0.210000 0.450000
0.210000 0.470000
0.210000 0.510000
0.210000 0.570000
0.210000 0.670000
0.210000 0.750000
0.230000 0.330000
0.230000 0.350000
0.230000 0.370000
0.230000 0.390000
0.230000 0.410000
0.230000 0.450000
0.230000 0.470000
0.230000 0.510000
0.230000 0.530000
0.230000 0.570000
0.230000 0.610000
0.230000 0.670000
0.230000 0.750000
0.250000 0.370000
0.250000 0.390000
0.250000 0.410000
0.250000 0.430000
0.250000 0.450000
0.250000 0.490000
0.250000 0.510000
0.250000 0.530000
0.250000 0.550000
0.250000 0.570000
0.250000 0.610000
0.250000 0.670000
0.250000 0.750000
0.270000 0.390000
0.270000 0.410000
0.270000 0.430000
0.270000 0.450000
0.270000 0.470000
0.270000 0.490000
0.270000 0.510000
0.270000 0.530000
0.270000 0.550000
0.270000 0.570000
0.270000 0.610000
0.270000 0.630000
0.270000 0.670000
0.270000 0.750000
0.290000 0.430000
0.290000 0.450000
0.290000 0.470000
0.290000 0.490000
0.290000 0.510000
0.290000 0.530000
0.290000 0.570000
0.290000 0.590000
0.290000 0.610000
0.290000 0.630000
0.290000 0.670000
0.290000 0.750000
0.310000 0.450000
0.310000 0.470000
0.310000 0.510000
0.310000 0.530000
0.310000 0.550000
0.310000 0.570000
0.310000 0.610000
0.310000 0.630000
0.310000 0.670000
0.310000 0.750000
0.310000 0.810000
0.330000 0.450000
0.330000 0.490000
0.330000 0.510000
0.330000 0.530000
0.330000 0.550000
0.330000 0.570000
0.330000 0.590000
0.330000 0.610000
0.330000 0.670000
0.330000 0.750000
0.330000 0.810000
0.350000 0.450000
0.350000 0.470000
0.350000 0.510000
0.350000 0.530000
0.350000 0.550000
0.350000 0.570000
0.350000 0.590000
0.350000 0.610000
0.350000 0.630000
0.350000 0.670000
0.350000 0.750000
0.350000 0.810000
0.370000 0.490000
0.370000 0.510000
0.370000 0.550000
0.370000 0.570000
0.370000 0.590000
0.370000 0.610000
0.370000 0.630000
0.370000 0.650000
0.370000 0.670000
0.370000 0.710000
0.370000 0.750000
0.370000 0.810000
0.390000 0.510000
0.390000 0.530000
0.390000 0.570000
0.390000 0.590000
0.390000 0.610000
0.390000 0.630000
0.390000 0.650000
0.390000 0.670000
0.390000 0.710000
0.390000 0.810000
0.390000 0.830000
0.410000 0.530000
0.410000 0.550000
0.410000 0.610000
0.410000 0.630000
0.410000 0.650000
0.410000 0.670000
0.410000 0.710000
0.410000 0.730000
0.410000 0.750000
0.410000 0.810000
0.410000 0.830000
0.430000 0.570000
0.430000 0.590000
0.430000 0.630000
0.430000 0.650000
0.430000 0.670000
0.430000 0.690000
0.430000 0.710000
0.430000 0.730000
0.430000 0.750000
0.430000 0.810000
0.450000 0.590000
0.450000 0.610000
0.450000 0.650000
0.450000 0.670000
0.450000 0.690000
0.450000 0.710000
0.450000 0.730000
0.450000 0.750000
0.450000 0.810000
0.450000 0.830000
0.450000 0.850000
0.470000 0.610000
0.470000 0.630000
0.470000 0.650000
0.470000 0.670000
0.470000 0.690000
0.470000 0.710000
0.470000 0.730000
0.470000 0.750000
0.470000 0.810000
0.470000 0.830000
0.470000 0.850000
0.490000 0.650000
0.490000 0.670000
0.490000 0.690000
0.490000 0.730000
0.490000 0.750000
0.490000 0.770000
0.490000 0.810000
0.490000 0.830000
0.490000 0.850000
0.510000 0.670000
0.510000 0.690000
0.510000 0.710000
0.510000 0.730000
0.510000 0.750000
0.510000 0.770000
0.510000 0.810000
0.510000 0.830000
0.510000 0.850000
0.510000 0.870000
0.530000 0.690000
0.530000 0.710000
0.530000 0.730000
0.530000 0.750000
0.530000 0.790000
0.530000 0.810000
0.530000 0.830000
0.530000 0.850000
0.530000 0.870000
0.550000 0.690000
0.550000 0.730000
0.550000 0.750000
0.550000 0.770000
0.550000 0.790000
0.550000 0.810000
0.550000 0.830000
0.550000 0.850000
0.550000 0.870000
0.570000 0.710000
0.570000 0.730000
0.570000 0.750000
0.570000 0.770000
0.570000 0.790000
0.570000 0.810000
0.570000 0.830000
0.570000 0.850000
0.570000 0.870000
0.590000 0.730000
0.590000 0.750000
0.590000 0.770000
0.590000 0.790000
0.590000 0.810000
0.590000 0.830000
0.590000 0.850000
0.590000 0.870000
0.590000 0.890000
0.610000 0.750000
0.610000 0.770000
0.610000 0.810000
0.610000 0.830000
0.610000 0.850000
0.610000 0.870000
0.610000 0.890000
0.610000 0.910000
0.630000 0.770000
0.630000 0.790000
0.630000 0.830000
0.630000 0.850000
0.630000 0.870000
0.630000 0.890000
0.630000 0.910000
0.650000 0.810000
0.650000 0.830000
0.650000 0.850000
0.650000 0.870000
0.650000 0.890000
0.650000 0.910000
0.670000 0.830000
0.670000 0.850000
0.670000 0.870000
0.670000 0.890000
0.670000 0.910000
0.690000 0.850000
0.690000 0.870000
0.690000 0.890000
0.690000 0.910000
0.710000 0.850000
0.710000 0.870000
0.710000 0.890000
0.710000 0.910000
0.710000 0.930000
0.730000 0.870000
0.730000 0.890000
0.730000 0.910000
0.730000 0.930000
0.750000 0.890000
0.750000 0.910000
0.750000 0.930000
0.770000 0.910000
0.770000 0.930000
0.770000 0.950000
0.790000 0.930000
0.790000 0.950000
0.810000 0.950000
0.830000 0.950000
0.850000 0.970000
};

==> points_list.tex <==
\addplot [only marks, mark=pentagon*, color=red] table {
0.030000 0.030000
0.030000 0.050000
0.030000 0.070000
0.050000 0.050000
0.050000 0.070000
0.050000 0.090000
0.070000 0.070000
0.070000 0.090000
0.070000 0.110000
0.090000 0.090000
0.090000 0.110000
0.090000 0.130000
0.090000 0.150000
0.110000 0.110000
0.110000 0.130000
0.110000 0.150000
0.110000 0.170000
0.110000 0.190000
0.130000 0.130000
0.130000 0.150000
0.130000 0.170000
0.130000 0.230000
0.150000 0.150000
0.150000 0.170000
0.150000 0.190000
0.150000 0.250000
0.150000 0.270000
0.170000 0.170000
0.170000 0.190000
0.170000 0.210000
0.170000 0.230000
0.170000 0.310000
0.190000 0.190000
0.190000 0.210000
0.190000 0.230000
0.190000 0.250000
0.190000 0.350000
0.210000 0.210000
0.210000 0.230000
0.210000 0.250000
0.210000 0.270000
0.210000 0.290000
0.230000 0.230000
0.230000 0.250000
0.230000 0.270000
0.230000 0.290000
0.230000 0.310000
0.230000 0.430000
0.250000 0.250000
0.250000 0.270000
0.250000 0.290000
0.250000 0.310000
0.250000 0.330000
0.250000 0.350000
0.250000 0.470000
0.270000 0.270000
0.270000 0.290000
0.270000 0.310000
0.270000 0.330000
0.270000 0.350000
0.270000 0.370000
0.290000 0.290000
0.290000 0.310000
0.290000 0.330000
0.290000 0.350000
0.290000 0.370000
0.290000 0.390000
0.290000 0.410000
0.290000 0.550000
0.310000 0.310000
0.310000 0.330000
0.310000 0.350000
0.310000 0.370000
0.310000 0.390000
0.310000 0.410000
0.310000 0.430000
0.310000 0.490000
0.310000 0.590000
0.330000 0.330000
0.330000 0.350000
0.330000 0.370000
0.330000 0.390000
0.330000 0.410000
0.330000 0.430000
0.330000 0.470000
0.330000 0.630000
0.350000 0.350000
0.350000 0.370000
0.350000 0.390000
0.350000 0.410000
0.350000 0.430000
0.350000 0.490000
0.370000 0.370000
0.370000 0.410000
0.370000 0.430000
0.370000 0.450000
0.370000 0.470000
0.370000 0.530000
0.390000 0.390000
0.390000 0.410000
0.390000 0.430000
0.390000 0.450000
0.390000 0.470000
0.390000 0.490000
0.390000 0.550000
0.390000 0.750000
0.410000 0.410000
0.410000 0.430000
0.410000 0.450000
0.410000 0.470000
0.410000 0.490000
0.410000 0.510000
0.410000 0.570000
0.410000 0.590000
0.430000 0.430000
0.430000 0.450000
0.430000 0.470000
0.430000 0.490000
0.430000 0.510000
0.430000 0.530000
0.430000 0.550000
0.430000 0.610000
0.430000 0.830000
0.450000 0.450000
0.450000 0.510000
0.450000 0.530000
0.450000 0.550000
0.450000 0.570000
0.450000 0.630000
0.470000 0.470000
0.470000 0.510000
0.470000 0.530000
0.470000 0.550000
0.470000 0.570000
0.470000 0.590000
0.490000 0.490000
0.490000 0.510000
0.490000 0.530000
0.490000 0.550000
0.490000 0.570000
0.490000 0.590000
0.490000 0.610000
0.490000 0.630000
0.490000 0.710000
0.510000 0.510000
0.510000 0.530000
0.510000 0.550000
0.510000 0.570000
0.510000 0.590000
0.510000 0.610000
0.510000 0.630000
0.510000 0.650000
0.530000 0.530000
0.530000 0.550000
0.530000 0.570000
0.530000 0.590000
0.530000 0.610000
0.530000 0.630000
0.530000 0.650000
0.530000 0.670000
0.530000 0.770000
0.550000 0.550000
0.550000 0.570000
0.550000 0.590000
0.550000 0.610000
0.550000 0.630000
0.550000 0.650000
0.550000 0.670000
0.550000 0.710000
0.570000 0.570000
0.570000 0.610000
0.570000 0.630000
0.570000 0.650000
0.570000 0.670000
0.570000 0.690000
0.590000 0.590000
0.590000 0.610000
0.590000 0.630000
0.590000 0.650000
0.590000 0.670000
0.590000 0.690000
0.590000 0.710000
0.610000 0.610000
0.610000 0.630000
0.610000 0.670000
0.610000 0.690000
0.610000 0.710000
0.610000 0.730000
0.610000 0.790000
0.630000 0.630000
0.630000 0.670000
0.630000 0.690000
0.630000 0.710000
0.630000 0.730000
0.630000 0.750000
0.630000 0.810000
0.650000 0.650000
0.650000 0.670000
0.650000 0.690000
0.650000 0.710000
0.650000 0.730000
0.650000 0.750000
0.650000 0.770000
0.650000 0.790000
0.670000 0.670000
0.670000 0.710000
0.670000 0.730000
0.670000 0.750000
0.670000 0.770000
0.670000 0.790000
0.670000 0.810000
0.690000 0.690000
0.690000 0.730000
0.690000 0.750000
0.690000 0.770000
0.690000 0.790000
0.690000 0.810000
0.690000 0.830000
0.710000 0.710000
0.710000 0.750000
0.710000 0.770000
0.710000 0.790000
0.710000 0.810000
0.710000 0.830000
0.730000 0.730000
0.730000 0.750000
0.730000 0.790000
0.730000 0.810000
0.730000 0.830000
0.730000 0.850000
0.750000 0.750000
0.750000 0.810000
0.750000 0.830000
0.750000 0.850000
0.750000 0.870000
0.770000 0.770000
0.770000 0.810000
0.770000 0.830000
0.770000 0.850000
0.770000 0.870000
0.770000 0.890000
0.790000 0.790000
0.790000 0.810000
0.790000 0.830000
0.790000 0.850000
0.790000 0.870000
0.790000 0.890000
0.790000 0.910000
0.810000 0.810000
0.810000 0.830000
0.810000 0.850000
0.810000 0.870000
0.810000 0.890000
0.810000 0.910000
0.810000 0.930000
0.830000 0.850000
0.830000 0.890000
0.830000 0.910000
0.830000 0.930000
0.850000 0.890000
0.850000 0.910000
0.850000 0.930000
0.850000 0.950000
0.870000 0.930000
};

==> points_none.tex <==
\addplot [only marks, mark=*, color=black] table {
0.690000 0.710000
0.730000 0.770000
0.750000 0.770000
0.830000 0.830000
0.830000 0.870000
0.850000 0.850000
0.850000 0.870000
0.870000 0.870000
0.890000 0.890000
0.910000 0.910000
0.930000 0.930000
0.950000 0.950000
0.970000 0.970000
0.990000 0.990000
};
